Characterizing Lifting and Lowering Activities with Insole FSR sensors in Industrial Exoskeletons

This paper presents an insole FSR (Force Sensing Resistor) to dynamically detect weight variations in an exoskeleton system. The proposed methodology is intended for tasks of lifting and lowering heavy weights with an industrial exoskeleton to substantially reduce spinal loads during these manual handling activities. Instead of extensively placing high-dense force sensors by covering the whole plantar area, as most of commercial applications do, we integrate only a few force sensors in specific plantar area, so that the sensory system is not restricted to an individual foot size and shape, and on the other hand has relatively lower material cost. Industrial exoskeletons are intended to assist workers when handling heavy goods. With this in mind, wearers are not able to use their hands to control the exoskeleton since they use them to handle the goods. Therefore, the exoskeleton controller is required to indirectly infer how much and when the wearer requires assistance for lifting or lowering a heavy weight. Our approach of dynamically detect and characterize the increment/decrement of weight, as well as the rising/falling edge, enables the exoskeleton's controller to trigger the request of assistive force to the actuators.

==> simulation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SECTION: SIMULATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%As described in the design section \ref{sec:design}, the optimal sensors arrangement must be able to easily differentiate force levels in the range of $8kg$ to $360kg$. %Also, we intent to integrate commercial thin film force sensors due to the small size as an external shoe platform.

%In order to verify our design, %, the sensors arrangement and analyze the force sensors responses to the different pressures. 
%we developed a simulation environment %, in which we are able to create a virtual force sensor from a equation or from a look up table resistance/force.
%In this way, we are able to simulate commercial sensors and select the best for our specific application. 
%Moreover, with the virtual environment it is possible to discretize the analog reading of the virtual force sensor and to apply a filter or amplifier to measure the resistance level, see figure \ref{figvirtualsensor}.

%The virtual force sensor is modeled by the equation \ref{eqvirtualforcesensor}

%\begin{equation}
%	f(y) =  \left(\frac{x}{R_1x^2+x}\right)
%	\label{eqvirtualforcesensor}
%\end{equation}

%\noindent where $y=resistance$, $x=force$ and a constant $R_1$ for a smooth curve-response, in this way the force response of the virtual sensor is similar to the data-sheets obtained from commercial sensors. 

%Also, it is possible able to model the virtual force sensor by applying a voltage divisor $V_{divisor}=Vcc(R_2/R_1+R_2)$, to the response function of the sensor $f(r) = 1/p$, where $r=resistance$ and $p=force$, where $R_1$ is the sensor resistance, $R_2$  is a fix resistor and $V_{cc}$ is a constant (voltage supply); with the proportions $R_2=200 \times R_1$ . %Similar to the equation \ref{eqvirtualforcesensor}, by adjusting $R_1$ it is possible to obtain similar response curves to model the resolution of the real force sensors, as shown in figure \ref{figvirtualsensor}.


%\begin{figure}[thpb]
%	\centering
%		\includegraphics[width=8.5cm]{figures/vs.png}
%		\caption{Virtual force sensor}
%		\label{figvirtualsensor}
%\end{figure}


Commercial thin film force sensors FSR have several drawbacks that make them not suitable for precise measurement of force. Their resistance response respect to the force is nonlinear and from sensor to sensor is different. This means that each sensor will respond with different resistance values even when the applied force is the same. 

Therefore, thin film FSR sensors require calibration and equalization when 2 or more sensors are plan to work together.

\subsection{Force Sensor Calibration} 

The FSR circuit to protect and obtain their force-resistance curves is shown in figure \ref{figforcesensorcalib}$a$. The circuit consists of a couple of voltage divisors. The first is a current limiter to $0.5mA$ which is the maximum current supported by the sensor \cite{shunt}, and it is also a voltage reducer from $5V$ to $3V$ to obtain a better resolution from the ADC (Analog to Digital Converter). The second voltage divisor is to obtain the readings from the FSR sensor. In this configuration, $R_2$ is calculated from the FSR resistance values averaging the higher and lower limits to obtain a considerable ratio to differentiate between the levels, see Table \ref{tbl:fsrtable}. 

%\begin{figure}[thpb]
%	\centering
%		\includegraphics[width=0.45\textwidth]{figures/figLfsensorsbreakADJUSTED.png}
%		\caption{Thin film FSR sensors with different responses to the same force ($0$ to $490N$) when loading/unloading with break.}
%		\label{the4sensorsbreak}
%\end{figure}

%\begin{figure}[thpb]
%	\centering
%		\includegraphics[width=0.45\textwidth]{figures/fig4sensorSLf.png}
%		\caption{Thin film FSR sensors with different responses to the same force ($0$ to $490N$)when loading/unloading continuosly.}
%		\label{the4sensorsNObreak}
%\end{figure}



\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/figLfsensorsbreakADJUSTED.png}
        \caption{Thin film FSR sensors with different responses to the same force ($0$ to $490N$) when loading/unloading with break.}
        \label{the4sensorsbreak}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/fig4sensorSLf.png}
        \caption{Thin film FSR sensors with different responses to the same force ($0$ to $490N$)when loading/unloading continuosly.}
        \label{the4sensorsNObreak}
    \end{subfigure}


   \caption{Insole FSR sensors calibration for the Left foot-front 
}\label{figleftfront}
\end{figure*}



In order to calibrate the FSR sensors we used a compression test machine, see figure \ref{figforcesensorcalib}$b$. We applied forces to each sensor in the range of 0 to 490N (50kg) in two different modalities. Loading continuos and loading with a break. When loading continuos the applied force is constantly increasing with steps of  of 98N (10kg) and retained for a couple of seconds from 0 to 490N and then decreasing back to 0N, see \ref{the4sensorsNObreak}. Similarly, when loading with a break, the force is applied in steps of 98N (10kg) and is hold for a couple of second, then the force is released, this process goes until the maximal range of 490N and the force is unloaded in the same way, as shown in figure \ref{the4sensorsbreak}.


\begin{table}[]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
Force level & R1  & R2  & Ratio  & Vout \\ 
(in N) & (FSR sensor) & (Fixed) & R2/(R1+R2) & (in V) \\ \hline
$490N$ (MAX)  & $500\Omega$             & $2.28k\Omega$      & 0.82               & 2.46V   \\ \hline
$200N$        & $3000\Omega$            & $2.28k\Omega$      & 0.43               & 1.29V   \\ \hline
$40N$ (min)   & $4000\Omega$            & $2.28k\Omega$      & 0.36              & 1.08V   \\ \hline
\end{tabular}
\caption{Voltage divisor values for FSR.}
\label{tbl:fsrtable}
\end{table}


The voltage readings from the FSR $V_{FSR}$ are converted to digital levels with an ADC (1024 steps of resolution). The voltage input $V_{IN} = 3V $, and the steps are calculated $Steps_{FSR} = V_{FSR} \times 1024 / V_{IN}$, see figures \ref{the4sensorsbreak},\ref{the4sensorsNObreak}.



\subsection{Force Sensor Equalization} 

Once the sensors are calibrated, their force-resistance curves are know. These curves reveals that the sensors are considerably different. 
And the next step is to equalize the curves, so the sensor can be treated as 'sensors with similar response'.

The equalization process is as follows: 
From all the sensor curves, the less sensible sensor is selected as the $base$ sensor to which all other sensors will try to match. 
In this context, the more sensible sensors are match to the $base$ sensor by adding compensation resistances in series to them. The resistance from a FSR sensor $R_{FSR} $ is obtained by Equation \ref{eq2}, where $R_2$ is the fix resistor in a voltage divisor configuration.

\begin{equation}
	R_{FSR} =  \left(\frac{V_{IN} R_2}{V_{IN} (Steps_{FSR}/ADC)}\right) - R2
	\label{eq2}
\end{equation}




The resistance levels from the FSR sensor are obtained and compared to the $base$ FSR. The average of the difference in resistances through the force levels (0 to 490N) is calculated per each FSR with respect to the $base$. And this difference is compensated by physical resistance to be added in series to the FSR to match the $base$ and be equalize. However, we can compensate the resistance level with software in the micro-controller to don't add the physical resistance.

\begin{figure}[thpb]
	\centering
		\includegraphics[width=0.45\textwidth]{figures/fig4x.jpg}
		\caption{FSR sensors equalization to responses ($0$ to $490N$). }
		\label{figforcesensorcalib}
\end{figure}



From our insole system, we equalized by foot two modules, the $front$ and $back$. To give an example: the $Left$ $front$ sensors, see figures \ref{the4sensorsbreak},\ref{the4sensorsNObreak} are equalized as follows:

The $base$ sensor is selected as the less sensible (with higher resistance overall the levels), we selected sensor $Lf2$. All other sensors from this module are adjusted to this $base$. The sensor resistances $Lf4_R$, $Lf3_R$ and $Lf1_R$ are subtracted to the $base$ sensor to obtain their compensation resistance to match the force-resistance curve from the $base$ sensor.

We obtained the compensation resistances from $LF2$: $Lf4_r=795.11\Omega$, $Lf3_r=658.76\Omega$ and $Lf1_r=127.44\Omega$ to be added in series by each FSR to be equalized to $Lf2$, resulting in a better force-resistance approximation, see figure \ref{sensorsequalized}.


\begin{figure}[thpb]
	\centering
		\includegraphics[width=0.45\textwidth]{figures/sensorsEqualized1st.png}
		\caption{$Lf1$, $Lf3$ and $Lf4$ FSR sensors equalization to the $base$ $Lf2$. }
		\label{sensorsequalized}
\end{figure}


\textbf{Discussion:} From a set of FSR sensors, the more sensible ones can be approximated to the less sensitive FSR. However, the force-resistance curves are still not the same. The best way to match the sensors is to equalize them to a specific range. In our equalization example we matched them to work in the range of $19.6N$ ($20kg$), see figure \ref{sensorsequalized}.



%\begin{figure*}[thpb]
%	\centering
%		\includegraphics[width=0.85\textwidth]{figures/sensorfusionok3.png}
		%\includegraphics[width=0.8\textwidth]{figures/sensorfusionok3.png}
%		\caption{Sensor fusion simulation. a) The control system registers the operator's body weight as $base$.  b) Operator lifting up: force sensors detecting the increment of weight (rising-edge) and the IMU detecting the inclination from bending position (falling-edge).  c) Operator lifting down: force sensors detecting the decrement of weight (falling-edge) and the IMU detecting the inclination from a standing position (rising-edge).}
%		\label{figsensorfusion}
%\end{figure*}


%In order to verify our design, we developed a simulation environment which is able to model commercial force sensors and simulate an industrial setting with a human operator, exoskeleton and different heavy goods. Additionally, in the simulator we included an IMU, to be integrated in the real setting in a sensor fusion scheme to control the industrial exoskeleton. 


% and to the virtual human to simulate the balancing when walking and lifting up/down heavy weight or on the contrary, have an ideal virtual setting without noise.
%------------------------------------------------------------------------------
% Subsection: Sensors configurations 
%------------------------------------------------------------------------------

\subsection{Sensor Configurations}
\label{senconf}

The proposed exoshoe design integrates eight force sensor per foot, making in total 16 force sensors. This means that ideally 16 input channels are required to monitor and process the sensors data from the feet. However, given the arrangement of sensors, it is possible to simplify the electronic circuit and cables by grouping the resistors (sensors) by each foot module, four sensors on the $front$ of the foot and four sensors on the $back$ of the foot. 

Important to mention is that the simplification of the electronic circuit is possible because of the equalization of the FSR sensors. Otherwise, the results from grouping the sensors will lead to erroneous data.

In this configuration, we studied and simulated to group the force sensors in parallel. We compare the results to the ideal case of taking into account the 16 sensors independently.%, see figure \ref{figsensorresis}.

\subsubsection{Independent sensors}

In the ideal case, the 16 sensors are processed independently, which means, each sensor is connected to a voltage divisor circuit, see figure \ref{figforcesensorcalib}$a$, to obtain a measurement in voltage $V(f)$ respect to received force $f$. The voltage measurement $f(V)$ is then translated to 1024 levels with an ADC and processed by the controller.  %In this way, the reading gives us the ground truth for our experiment. 

%\subsubsection{Sensors in series}

%In order to simplify the data channels, the 16 sensors are divided in four groups, two sets per foot. Where, each group add the four sensor-resistances in series $Rs_{left_{top}}=R_{left_1}+R_{left_2}+R_{left_3}+R_{left_4}$ (the same for $Rs_{left_{back}}$, $Rs_{right_{top}}$ and $Rs_{right_{back}}$), see figure \ref{figsensorresis}$c$. 

%The results from this approach shows an increment in the resistance per group resulting in a fraction of the applied force. In other words, the sum of resistances divides the total weight reducing the scale of the sensors.%Thus, the sensors in series basically reduce the scale of the . 




\subsubsection{Sensors in parallel}

The 16 sensors are divided in four modules. Each module adds their corresponding four sensor-resistances in parallel: $1/R_{module} = 4\times1/R_{individual}$. 
Where $R_{module}$ is the resistance of 4-sensors group and $R_{individual}$ is the resistance of each force sensor.
%$1/Rp_{left_{top}}=1/R_{left_1}+1/R_{left_2}+1/R_{left_3}+1/R_{left_4}$ (the same for $Rp_{left_{back}}$, $Rp_{right_{top}}$ and $Rp_{right_{back}}$), see figure \ref{figsensorresis}$d$.


\textbf{In the simulation:} 
The results from adding resistances in parallel are the same to the sum of individual force sensors. Thus, the insole complexity per foot can be reduced from 8 to 2 data channels.




%\begin{figure*}[thpb]
%	\centering
%		\includegraphics[width=\textwidth]{figures/sensorsarrangement.png}
%		\caption{Results from adding force sensors. a) Independently. b) Series. c) Parallel.}
%		\label{figaddforcesensors}
%\end{figure*}


%------------------------------------------------------------------------------
% Subsection: Exoskeleton simulation 
%------------------------------------------------------------------------------

%\subsection{Exoskeleton Simulation}

%With the simulation environment it is possible to observe the behavior of the force sensors and IMU together in a sensor fusion scheme. As mentioned before, the exoshoe detects the weight variation of the operator, while the IMU detects the angle of the operator's back. 
%The simulation results show the correlation of angle (operator's inclination) with the increment/decrement of weight as a signal edge. When a rising-edge is detected in the force sensors and a falling-edge is registered by the IMU, this means that the operator is lifting up the load. While, when falling-edge on the weight and rising-edge on the IMU occur, then the operator is lowering the load, see figure \ref{figsensorfusion}.


%Hence, with the sensor fusion technique we can infer when the operator is lifting up or down a weight by analyzing the data of both sensors, the force sensors and the IMU.



	
	

